Tensor-on-tensor Regression Neural Networks for Process Modeling with High-dimensional Data

Modern sensing and metrology systems now stream terabytes of heterogeneous, high-dimensional (HD) data profiles, images, and dense point clouds, whose natural representation is multi-way tensors. Understanding such data requires regression models that preserve tensor geometry, yet remain expressive enough to capture the pronounced nonlinear interactions that dominate many industrial and mechanical processes. Existing tensor-based regressors meet the first requirement but remain essentially linear. Conversely, conventional neural networks offer nonlinearity only after flattening, thereby discarding spatial structure and incurring prohibitive parameter counts. This paper introduces a Tensor-on-Tensor Regression Neural Network (TRNN) that unifies these two paradigms.

==> old_intro.tex <==
The advancement of sensing and metrology systems offers various opportunities in modern applications, particularly in the fields of additive and smart manufacturing \citep{gibson2021design}. Modern technology allows enormous amount of measurements to be taken over the manufacturing, chemical and other processes, facilitating the process modeling and monitoring. These processes are equipped with either massive number of sensors to generate rich functional data streams such as sensor signals \citep{lei2010automatic, yan2018real}, image sensing systems to either take snapshots of products every pre-set time intervals during the process or take one at the end of production \citep{jin2000identification,prasath2013comparison,yan2017anomaly}, or with advanced metrology instruments such as coordinate measuring machines (CMM) with touch probe or laser scanners to produce high density point clouds \citep{yan2019structured}. The large amount of measurements, either in the form of profiles, images or point clouds, are usually referred to as high dimensional (HD) data. The collected HD data are generated from heterogeneous sources, each set representing the behavior of certain part of the underlying system. Complex relationships can exist among multiple data sources, within which some belong to predictors related to process parameters and machine settings, and others belong to responses like manufactured product shapes. Modeling the association between these heterogeneous HD data has the potential to benefit a number of applications. For example, in the lithographic process of semiconductor manufacturing, the corrections of wafer overlay error could be made beforehand based on the error prediction from the wafer shape, which requires an image-on-image regression model \citep{turner2013role}. In the turning process, the machining parameters can influence the response surfaces of manufactured parts \citep{pacella2018multilinear}. The average point clouds of cylinder parts manufactured under different cutting speeds and cutting depths are shown in Figure \ref{fig:case1plot}. In materials science, models between the microstructure images of the material and the operating conditions signals like pressure/temperature are constructed \citep{khosravani2017development,gorgannejad2019quantitative}. Other applications include food production \citep{yu2003multivariate} and healthcare \citep{bellon1995experimental, balageas2010structural}. \\

\begin{figure}[htbp]
\includegraphics[scale=0.5]{case1plot.png}
\centering
\caption{\label{fig:case1plot} Examples of average cylinders under different cutting conditions}
\end{figure}

 Various research have been conducted in the literature with a focus on the regression analysis of scalars or one-dimensional functional data like profiles, waveform signals, longitudinal or stock data. Vanilla linear regression method treats each covariate in the data independently, which can lead to severe overfitting problem for HD data because of the excessive number of regressors comparing to the number of samples. The ignorance of the correlations among the predictors is alleviated by principal component regression (PCR) and partial least squares (PLS) by projecting the HD data into low dimensional subspaces. Further development of the methodology leads to functional data analysis, with a special focus on functional regression model (FRM) recently \citep{liang2003relationship,ramsay2008functional,yao2005functional,reiss2010fast,fan2014functional,ivanescu2015penalized,luo2017function}. It is capable of capturing nonlinear correlation structures between profiles with its built-in data reduction mechanism. The issue is that most of the FRM approaches assume knowing the basis functions from the engineers' domain knowledge and fail to be data-driven. To address this drawback, \citep{luo2017function} proposed a functional-on-functional regression method that can self-learn the basis functions from data. However, all the above approaches fail to generalize in a straightforward and effective way to more complex data like images and point clouds, which potentially containing richer system information. Although these complex forms of data can be flattened into one-way vectors, directly applying the methods fails to exploit their spatial structure.\\ 
 
 The difficulty should be overcome in the modeling of the complex forms of HD data including images and point clouds. \cite{colosimo2011analyzing} tackled the difficulty by projecting the HD point clouds into PC scores using the innovative complex PCA first before applying multivariate ANOVA to analyze the effects of machining variables on the projected scores. The main drawback of this approach is the ignorance of the interrelationship between process variables and point clouds, resulting from the separation of the dimension reduction and modeling steps. Tensor analysis, due to its ability to reduce the data dimension while capturing the underlying spatial structure, has been employed in the many areas including network analysis, process modeling and anomaly detection \citep{sun2006window, sapienza2015detecting, yan2014image}. Images and structured point clouds are measured on prespecified grids. Enjoying their grid structure, they can be compactly represented as tensors. Tensor techniques have been well explored in their regression models in the literature to handle the high dimensionality issue of estimated parameters. The first category of methods models a scalar response as a function of tensor covariates. \cite{zhou2013tensor} proposed to predict a scalar response from an image tensor by performing CP decomposition \citep{kiers2000towards}. They subsequently extended it using a generalized linear model for the response to have exponential family properties. \cite{li2018tucker} developed a scalar-on-tensor regression framework using Tucker decomposition \citep{tucker1963implications} as the dimensional reduction technique instead. The second category of models have a tensor response and scalar predictors. \cite{li2011multiscale} chose to build a regression model for each entry in the tensor response and fitted a parametric map eventually on the regression coefficients over the tensor. Nevertheless, the independent treatment of the response entries neglects the underlying spatial structure. A parsimonious linear tensor regression model is proposed to compensate this issue assuming the response tensor is sparse \citep{li2017parsimonious}. However, this assumption is limited to its neuroimaging application. \cite{yan2019structured} noticed that the HD point cloud tensor has intrinsic low-dimensional structure and applied low-dimensional basis to significantly reduce the number of parameters needed for estimation. The basis functions can be either prespecified or derived in a data-driven way. \\

The above two categories of tensor regression approaches only serve when one of the input or the output is a scalar variable. More generalized methods are discussed in the literature performing tensor-on-tensor regression. \cite{bro1996multiway} generalized PLS to N-way PLS (N-PLS) by applying CP decomposition to find the best subspaces to explain the variance between the input and output tensors. The performance of N-PLS, however, is diminished by its poor expression power, high complexity and slow convergence speed when tensors have order greater than 3. Higher-order partial least squares (HOPLS) solved this problem using Tucker decomposition instead to allow more model complexity and flexibility \citep{zhao2012higher}. Nevertheless, the computation of the covariance tensor is extremely inefficient and sometimes even intractable. The tensor-on-tensor (TOT) regression framework avoids dealing with the covariance tensor by learning the basis functions automatically from data \citep{lock2018tensor}. The major weakness is that the CP decomposition used in the method requires the input and output bases to have the same rank. At the same time, its high space complexity limits its tractability on large tensors. \cite{gahrooei2021multiple} developed a multiple tensor-on-tensor (MTOT) regression approach to unify the estimation of scalar, profile, image, or structured point cloud from heterogeneous HD data. In this way the input and output tensors are free to have different ranks.\\

However, the approaches described above are still restricted by the assumption of the linear relationship between input and output tensors. These approaches more or less reply on tensor techniques like CP and Tucker decompositions, which are still linear methods though dealing with high order tensors. In the real world, more complex nonlinear relationship often presents between sources and responses. In this regard, neural networks is a powerful tool in the literature to capture their nonlinear linkage. Neural networks grows increasingly popular in recent years, due to its overwhelming competence in modeling sophisticated relationship where most statistical methods fail. Though originally working on vectors, the neural networks has been extended to work on tensors by a number of papers. For example, \cite{liu2016tensor} developed a novel nonlinear tensor decomposition method using variational auto-encoder. \cite{li20213d} constructed a 3D tensor auto-encoder with special applications on video compression, while \cite{qian2021dtae} proposed a deep tensor auto-encoder structure for tensor completion purposes of the 3D seismic data. Despite of lots of approaches with similar names with ours, only two can be found in the literature that are relevant to our work. \cite{chien2017tensor} developed a classification neural networks that can accept tensor inputs. However, this approach only focused on the classification problem with scalar responses, and cannot apply to our regression case where both input and output are tensors of possible different orders. \cite{kossaifi2017tensor} managed to alleviate the problem in the convolutional neural networks that the flattening operation on the tensor before fully connected layers ignores the tensor's underlying spatial structure. Though proposed similar layers with ours, they aimed to solve the completely different problem. Thus, due to much difference in the network structure, their method cannot be directly applied to our tensor-on-tensor regression problem. Although flattening the tensor into a vector and consequently utilizing vanilla neural networks is one naive way to tackle the problem, it leads to too many parameters for training and is incapable of capturing the multi-linear structure of the tensor. \\

